Designing High-Performing Networks for Multi-Scale Computer Vision

Since the emergence of deep learning, the computer vision field has flourished with models improving at a rapid pace on more and more complex tasks. We distinguish three main ways to improve a computer vision model: (1) improving the data aspect by for example training on a large, more diverse dataset, (2) improving the training aspect by for example designing a better optimizer, and (3) improving the network architecture (or network for short). In this thesis, we chose to improve the latter, i.e. improving the network designs of computer vision models. More specifically, we investigate new network designs for multi-scale computer vision tasks, which are tasks requiring to make predictions about concepts at different scales. The goal of these new network designs is to outperform existing baseline designs from the literature. Specific care is taken to make sure the comparisons are fair, by guaranteeing that the different network designs were trained and evaluated with the same settings. Code is publicly available at https://github.com/CedricPicron/DetSeg.

==> chapters/abstract/abstract.tex <==

\chapter{Abstract} \label{ch:abstract}

Since the emergence of deep learning, the computer vision field has flourished with models improving at a rapid pace on more and more complex tasks. We distinguish three main ways to improve a computer vision model: (1) improving the data aspect by for example training on a large, more diverse dataset, (2) improving the training aspect by for example designing a better optimizer, and (3) improving the network architecture (or network for short). 

In this thesis, we chose to improve the latter, \ie improving the network designs of computer vision models. More specifically, we investigate new network designs for multi-scale computer vision tasks, which are tasks requiring to make predictions about concepts at different scales. The goal of these new network designs is to outperform existing baseline designs from the literature. Specific care is taken to make sure the comparisons are fair, by guaranteeing that the different network designs were trained and evaluated with the same settings.

The dissertation starts off by outlining the research setting and by formulating our general research goal in Chapter~\ref{ch:introduction}. The thesis proceeds by laying the foundations of our research setting in Chapter~\ref{ch:background}, where we introduce the backbone-neck-head meta architecture and describe the tasks, datasets, metrics, and standardized deep learning settings used throughout the thesis. In following chapters, we propose a couple of new high-performing network designs for multi-scale computer vision tasks, and make some interesting observations along the way.

In Chapter~\ref{ch:neck}, we introduce our own neck design called Trident Pyramid Network (TPN). Different from existing necks such as BiFPN, the TPN neck contains hyperparameters allowing to balance the communication-based processing and self-processing within the neck. Experiments show that these hyperparameters enable a better balance, yielding increased object detection performance as a result. Additionally, we empirically show that it is more beneficial to add computation to the neck part of the meta architecture, rather than to the backbone or head part. This result could have far-reaching consequences for the computer vision field, with its current and possibly unjustified strong focus on backbone networks.

In Chapter~\ref{ch:detection}, we design our own object detection heads called FQDet and FQDetV2. The FQDet heads are query-based two-stage object detection heads, which combine the best of both classical and DETR-based detectors. Among other things, the FQDet heads successfully introduce the use of anchors into the query-based paradigm, increasing the resulting bounding box accuracies and improving the network convergence speeds. Additionally, we also introduce the static top-k matching scheme producing stable assignments from the start of training, leading to even faster convergence, especially when compared to the dynamic Hungarian matching scheme. Following a series of controlled design experiments, we improve the FQDet in various ways resulting in the FQDetV2 head. Most notably, we observe that increasing the number of queries can lead to significant performance gains at a limited computational cost.

In Chapter~\ref{ch:segmentation}, we introduce our own segmentation head called EffSeg. The EffSeg head performs fine-grained instance and panoptic segmentation in an efficient way, thanks to our novel Structure-Preserving Sparsity (SPS) method. As opposed to performing computation in all locations of a dense 2D feature map, the SPS method allows to only process a specific set of feature locations (called active feature locations), in order to efficiently obtain fine-grained segmentation masks. The SPS method achieves this by separately storing the active feature, the passive features, and a dense 2D index map storing the feature indices such that any 2D operation in active feature locations can still be performed. By leveraging the SPS method, the EffSeg head obtains excellent segmentation performance at a significantly reduced computational cost compared to the baseline segmentation heads.

In Chapter~\ref{ch:conclusion}, we conclude our dissertation by summarizing our thesis and by highlighting our main contributions. Finally, we also discuss the main limitations of our work and provide directions for future research.

\cleardoublepage


==> chapters/abstractnl/abstractnl.tex <==
\chapter{Beknopte samenvatting}

Sinds de opkomst van diep leren is het computervisie veld aanzienlijk gegroeid met modellen die verbeteren aan een verschroeiende snelheid op steeds complexere taken. We onderscheiden volgende drie voornaamste manieren om een computervisie model te verbeteren: (1) het verbeteren van het data gedeelte door bijvoorbeeld te trainen op een grote, meer diverse dataset, (2) het verbeteren van het training gedeelte door bijvoorbeeld een betere optimalisator te ontwerpen en (3) het verbeteren van de netwerk architectuur (of netwerk in het kort).

In deze thesis kozen we ervoor om dit laatste te verbeteren, d.w.z. het verbeteren van netwerkontwerpen voor computervisie modellen. Meer bepaald onderzoeken we nieuwe netwerkontwerpen voor meer-schalige computervisie taken, hetgeen taken zijn die voorspellingen moeten maken voor concepten van verschillende schalen. Het doel van deze nieuwe netwerkontwerpen is om bestaande referentie ontwerpen uit de literatuur te overtreffen. Hierbij zorgen we ervoor dat de gemaakte vergelijkingen eerlijk zijn, door te garanderen dat de verschillende netwerkontwerpen getraind en geëvalueerd zijn met dezelfde instellingen.

Het proefschrift begint met het situeren van het onderzoek en met het formuleren van ons algemeen onderzoeksdoel in Hoofdstuk~\ref{ch:introduction}. Vervolgens leggen we de basisbeginselen vast voor het onderzoek in Hoofdstuk~\ref{ch:background}, waarbij we de rug-nek-hoofd meta architectuur introduceren en de taken, datasets, metrieken en gestandaardiseerde diep leren instellingen beschrijven. In de volgende hoofdstukken stellen we een aantal nieuwe hoog-performante netwerkontwerpen voor voor meer-schalige computervisie taken en maken we gaandeweg een aantal interessante observaties.

In Hoofdstuk~\ref{ch:neck} introduceren we ons eigen nek ontwerp Trident Pyramid Networks (TPN) genaamd. Verschillend van bestaande nekken zoals BiFPN, bevat de TPN nek hyperparameters die toelaten om de communicatie-gebaseerde berekeningen en de zelf-berekeningen te balanceren binnen de nek. Experimenten tonen aan dat deze hyperparameters voor een beter evenwicht (kunnen) zorgen, met betere objectdetectie performantie als resultaat. Bovendien tonen we empirisch aan dat het voordeliger is om extra rekenkracht toe te voegen aan het nek gedeelte van de meta architectuur, eerder dan aan het rug of hoofd gedeelte. Dit resultaat zou verreikende gevolgen kunnen hebben voor het computervisie veld, omwille van zijn huidige en potentieel ongegrond sterke focus op rug netwerken.

In Hoofdstuk~\ref{ch:detection} ontwerpen we onze eigen objectdetectie hoofden FQDet en FQDetV2 genaamd. De FQDet hoofden zijn vraag-gebaseerde tweetraps objectdetectie hoofden die het beste van klassieke en DETR-gebaseerde hoofden combineert. De FQDet hoofden introduceren o.a. met succes het gebruik van ankers in het vraag-gebaseerde paradigma, met accuratere begrenzingsvakken en snellere convergentie als gevolg. Daarnaast introduceren we ook het statische top-k koppeling schema dat stabiele toekenningen produceert sinds de start van het trainen, met betere convergentie tot gevolg, zeker wanneer vergeleken wordt met het dynamische Hongaars koppeling schema. Na een reeks gecontroleerde experimenten, slagen we erin het FQDet hoofd verder te verbeteren, hetgeen resulteert in het FQDetV2 hoofd. Als voornaamste bijdrage merken we op dat het vergroten van het aantal vragen leidt tot een significante verbetering in performantie aan een beperkte computationele kost.

In Hoofdstuk~\ref{ch:segmentation} introduceren we ons eigen segmentatie hoofd EffSeg genaamd. Het EffSeg hoofd voert fijn-korrelige instantie en panoptische segmentatie uit op een efficiënte manier dankzij onze nieuwe Structure-Preserving Sparsity (SPS) methode. In tegenstelling tot berekeningen uit te voeren op alle locaties in een dichtbezette 2D kenmerkenkaart, laat de SPS methode toe om enkel een specifieke groep van kenmerk locaties (actieve kenmerk locaties genaamd) te verwerken, om zo op een efficiënte wijze fijn-korrelige segmentatie maskers te bekomen. De SPS methode bereikt dit door het apart opslaan van actieve kenmerken, passieve kenmerken, en een dichtbezette 2D index kaart die de kenmerk indices opslaat zodanig dat om het even welke 2D operatie nog steeds uitgevoerd kan worden in actieve kenmerk locaties. Dankzij de SPS methode behaalt het EffSeg hoofd uitstekende segmentatie performantie aan een significant lagere computationele kost vergeleken met de referentie hoofden.

In Hoofdstuk~\ref{ch:conclusion} concluderen we ons proefstuk door onze thesis samen te vatten en door onze voornaamste bijdragen op te sommen. Ten slotte, bespreken we ook de voornaamste beperkingen van ons werk en geven we aanwijzingen voor verder onderzoek.

\cleardoublepage


==> chapters/curriculum/curriculum.tex <==
\chapter{Curriculum} \label{ch:curriculum}

Cédric Picron was born in Brussels (Belgium) in 1996. In 2017, he completed his bachelor's degree at the Vrije Universiteit Brussel (VUB) graduating in Electrical Engineering, and in 2019, he completed his master's degree at the KU Leuven graduating in Mathematical Engineering. Later that year, he joined the Processing Speech and Images (PSI) research group at KU Leuven as a PhD candidate, under supervision of Prof. Tinne Tuytelaars. His research focuses on designing high-performing networks for multi-scale computer vision tasks, such as object detection and segmentation.

During his PhD, he contributed to the university's teaching activities by giving exercise sessions and correcting exam questions for the `Digitale elektronica en processoren’ course, and by supervising following master theses:

\begin{itemize}
    \vspace{-0.2cm}
    \setlength\itemsep{0em}
    \item \textit{Monocular Pose Estimation of Vehicles in Traffic based on Deep Metric Learning}, Georgios Kouros (2021).
    \item \textit{Custom Tag Detection on an Unmanned Aerial Vehicle}, Gaétan Paul (2021-2022).
\end{itemize}

\cleardoublepage


==> chapters/preface/preface.tex <==
\chapter*{Preface} \label{ch:preface}

This is it. The end of four years (and a couple of months) of research. A journey with ups and downs, though the many paper rejections make me look back on my PhD with mixed feelings.

My most fond memory as a researcher, was when I got the results of my first FQDetV2 experiments. I had been running some controlled experiments trying to improve the FQDet head, meticulously testing different settings and variations one by one. I had found different promising improvements, but never tested them combined. I hence combined the improvements, coined the new head FQDetV2, and ran experiments to evaluate its performance. It felt like designing different parts of a spaceship, adding them to the ship, and hoping the whole would work, knowing that each part individually works flawlessly. When, on a Saturday morning, I got the results, I was ecstatic. The FQDetV2 head not only surpassed my expectations, but also outperformed the state-of-the-art (SOTA) object detection head at the time. The object detection benchmark on COCO is one of the most competitive benchmarks in the field. Reaching SOTA performance is hence far from easy (there can only be one the best), and I had never imagined my designs ever would be close to SOTA, let alone surpass it. Of course, critics might say this is just a number, but these numbers are currently the best way we have to evaluate object detection models. In the meanwhile, a new SOTA object detection head has emerged slightly surpassing FQDetV2, but with some small improvements FQDetV2 might come out on top (\textit{hoop doet leven}).

My research journey was also characterised with occasional downs, mostly due to paper rejections. Throughout my PhD, I submitted $13$ times to various conferences, and got accepted $3$ times. An acceptance ratio of 23\%. None of my papers got accepted in the first two times of asking. Given that review cycles can take many months, months sometimes years pass without paper publication, while in the meantime new works get published, rendering paper acceptance even harder as time goes by. The reasons for rejection were often vague, with reviewers often claiming a lack of novelty to justify their weak reject rating. Arguing in the rebuttal against the arguments put forward by the reviewers, felt like punching against a brick wall (\textit{it ain't gonna move}). A waste of time if you ask me. I hope the reviewing process will improve in the future, because all a researcher sometimes needs, is a little bit of recognition from the community.

Despite these setbacks, I always got the support of my supervisor Tinne, for which I will never be able to thank her enough. I remember her writing me an email on a Saturday morning to console me after poor paper reviews for one of my first papers, a kind gesture which made me feel better. I also thank her for giving me the opportunity to work on my own projects and pursuing my own interests, at a time when I was not motivated to continue working on the Ford project. I wish I could have published more papers at high-tier conferences to thank her for her trust, but unfortunately that did not happen. I enjoyed our regular meetings where I could share my new ideas and results. It always amazed me how easily she could follow my ideas and how well she remembered them for the next meeting, especially considering she has around a dozen of PhD students working on various topics. Thank you Tinne for taking such good care of your PhD students.

Next, I would like to thank the many exceptional people from our lab that I have met throughout my PhD. I would like to thank my office mates Tim Lebailly and Dušan for the many great discussions we have had (even though I was not often there). I would like to thank Paul for diligently organizing all of our trips, and Bert for taking such good care of our compute infrastructure.

The summer school and conference trips were definitely one of the highlights of my PhD. I would like to thank Timm Heß, Gorjan, Teodora, Dina, and Viktor for the great moments we have shared in Gran Canaria, Georgios and Eli for the great memories from London, and Tim Lebailly, Georgios, Simen, Gorjan, Dušan, Teodora, and Abhishek for the great times in Paris.

Finally, I would like to thank my family and friends for their everyday support, and especially my parents and my brother Loïc.

\cleardoublepage


==> chapters/publications/publications.tex <==
\chapter{Publications} \label{ch:publications}

\section*{Conference proceedings}

\begin{itemize}
    \item \bibentry{picron2021my}
    \item \bibentry{picron2022trident}
    \item \bibentry{picron2022fqdet}
\end{itemize}

\section*{Pre-prints}
\begin{itemize}
    \item \bibentry{picron2023effseg}
\end{itemize}

\cleardoublepage

